Improving the Regularity of Vector Fields

Let $\alpha>0$, $\beta>\alpha$, and let $X_1,\ldots, X_q$ be $\mathscr{C}^{\alpha}_{\mathrm{loc}}$ vector fields on a $\mathscr{C}^{\alpha+1}$ manifold which span the tangent space at every point, where $\mathscr{C}^{s}$ denotes the Zygmund-H\"older space of order $s$. We give necessary and sufficient conditions for when there is a $\mathscr{C}^{\beta+1}$ structure on the manifold, compatible with its $\mathscr{C}^{\alpha+1}$ structure, with respect to which $X_1,\ldots, X_q$ are $\mathscr{C}^{\beta}_{\mathrm{loc}}$. This strengthens previous results of the first author which dealt with the setting $\alpha>1$, $\beta>\max\{ \alpha, 2\}$.

==> Further.tex <==
We do not know whether there is a quantitative result for $\beta\in(0,1]$, because when $X_1,\dots,X_n\in\Co^\beta$ the exponential map $\Phi(t)=e^{t^1X_1+\dots +t^nX_n}p $ may not be defined for $\beta<1$ and do not have the $\Co^\beta$-regularity. Also we may need to find a suitable definition of $\Co^{\beta-1}_X$-norm for functions and differential forms, as throughout the paper we only define $\Co^{\beta-1}_{X,\loc}(\Manifold)$ but not $\Co^{\beta-1}_{X}(\Manifold)$.

%We do not know how to prove $\ZygVF\beta X\neq\Co^\beta_{X,\loc}$ for 2-forms and higher order forms.

% We do not know how to prove Proposition \ref{Prop::FuncVF::ZygVFInVSHas} if we remove the assumption $\alpha>\frac12$.
% \begin{prob}Let $\alpha\in(0,\frac12]$ and let $\beta\in(1-\alpha,\alpha+1]$. Let $X_1,\dots,X_n\in\Co^\alpha(\Ball^n;T\Ball^n)$ that spans the tangent spaces at every point. 

% Suppose $\omega\in\Co^{\beta-1}(\Ball^n;\mywedge^kT^*\Ball^n)$ satisfies $d\IntProd{X_1}d\omega,\dots,d\IntProd{X_n}d\omega\in \Co^{\beta-2}(\Ball^n;\mywedge^{k+1}T^*\Ball^n)$. Do we must have $d\omega\in \Co^{\beta-1}(\Ball^n;\mywedge^{k+1}T^*\Ball^n)$?
% \end{prob}


The canonical coordinates (exponential map) may not produce the sharp pullback regularity for the given vector fields collection.
